Low-energy lepton physics in the MRSSM: $(g-2)_\mu$, $\mu \to e\gamma$ and $\mu\to e$ conversion

Low-energy lepton observables are discussed in the Minimal R-symmetric Supersymmetric Standard Model. We present comprehensive numerical analyses and the analytic one-loop results for $(g-2)_\mu$, $\mu \to e \gamma$, and $\mu \to e$ conversion. The interplay between the three observables is investigated as well as the parameter regions with large $g-2$. A striking difference to the MSSM is the absence of $\tan\beta$ enhancements; however we find smaller enhancements governed by MRSSM-specific R-Higgsino couplings $\lambda_d$ and $\Lambda_d$. As a result we find significant contributions to $g-2$ only in a small parameter space with several SUSY masses below $200$ GeV, compressed spectra and large $\lambda_d$, $\Lambda_d$. In this parameter space there is a correlation between all three considered observables. In the parameter region with small $(g-2)_\mu$ the SUSY masses can be larger and the correlation between $\mu\to e\gamma$ and $\mu\to e$ conversion is weak. Therefore already COMET Phase 1 has a promising sensitivity to the MRSSM.

==> MuE.tex <==
\section{$\mu \to e$ coherent conversion in nuclei} 
Our starting point is the eq.~14 in \cite{Kitano:2002mt}
\begin{equation}
  \omega = 2 G_F^2 \left|- \frac{\sqrt{2}}{8 G_F} A_2^L D + \tilde{g}^{(p)}_{LS} S^{(p)} + \tilde{g}^{(n)}_{LS} S^{(n)} + \tilde{g}^{(p)}_{LV} V^{(p)} + \tilde{g}^{(n)}_{LV} V^{(n)}\right|^2 + L \leftrightarrow R
\end{equation}
where
\begin{align}
  \tilde{g}^{(a)}_{LS,RS} = & \sum_q G_S^{q,a} g_{LS,RS,q} \\
  \tilde{g}^{(p)}_{LV,RV} = & 2 g_{LV,RV(u)} + g_{LV,RV(d)} \\
  \tilde{g}^{(n)}_{LV,RV} = & g_{LV,RV(u)} + 2 g_{LV,RV(d)}
\end{align}
with the normalization of coupling in eq. 1 thereof as 
\begin{eqnarray}
    {\cal L}_{\rm int} &=&
    - \frac{4 G_{\rm F}}{\sqrt{2}}
    \left(
    m_\mu A_R \bar{\mu} \sigma^{\mu \nu} P_L e F_{\mu \nu}
    + m_\mu A_L \bar{\mu} \sigma^{\mu \nu} P_R e F_{\mu \nu}
    + {\rm h.c.}
    \right) \nonumber \\
    &&
    - \frac{G_{\rm F}}{\sqrt{2}} \sum_{q = u,d,s}
    \left[ {\rule[-3mm]{0mm}{10mm}\ } \right.
    \left(
    g_{LS(q)} \bar{e} P_R \mu + g_{RS(q)} \bar{e} P_L \mu
    \right) \bar{q} q  \nonumber \\
    &&   \hspace*{2.4cm}
    +
    \left(
    g_{LP(q)} \bar{e} P_R \mu + g_{RP(q)} \bar{e} P_L \mu
    \right) \bar{q} \gamma_5 q \nonumber \\
    &&   \hspace*{2.4cm}
    +
    \left(
    g_{LV(q)} \bar{e} \gamma^{\mu} P_L \mu
    + g_{RV(q)} \bar{e} \gamma^{\mu} P_R \mu
    \right) \bar{q} \gamma_{\mu} q \nonumber \\
    &&   \hspace*{2.4cm}
    +
    \left(
    g_{LA(q)} \bar{e} \gamma^{\mu} P_L \mu
    + g_{RA(q)} \bar{e} \gamma^{\mu} P_R \mu
    \right) \bar{q} \gamma_{\mu} \gamma_5 q \nonumber \\
    &&   \hspace*{2.4cm}
    + \ \frac{1}{2}
    \left(
    g_{LT(q)} \bar{e} \sigma^{\mu \nu} P_R \mu
    + g_{RT(q)} \bar{e} \sigma^{\mu \nu} P_L \mu
    \right) \bar{q} \sigma_{\mu \nu} q
	+ {\rm h.c.}
    \left. {\rule[-3mm]{0mm}{10mm}\ } \right]\ ,
    \label{1}
\end{eqnarray}
The relation between photonic dipoles in Fok \& Kribs and Kitano $A^{L/R}_{\gamma dip}$, Koike \& Okada $A_{L/R}$ and \texttt{Flavorkit}  is the following
\begin{equation}
  \frac{1}{2} A^{L/R}_{\gamma dip} = -\frac{4 G_\mu}{\sqrt{2}} A_{L/R}^* = \frac{1}{2} K_2^{L/R}
\end{equation}
Therefore there's a sign difference.
while \texttt{SPheno} uses

The eq.~58 in \cite{Hisano:1995cp} can be obtained from \cite{Kitano:2002mt} by a set of approximations
\begin{align}
  \Phi^2 = & 4 m_\mu^3 \alpha^3 Z_{eff}^4/Z \\
  S_p = & \frac{1}{8\pi} m_\mu \Phi Z F_p & \\
  S_n = & \frac{N}{Z} S_p \\
  V_P = & S_p\\
  V_n = & \frac{N}{Z} V_p \\
  D = & 8 e V_p
\end{align}  
Factors of $N/Z$ follow from eq. 20 - 23 in \autocite{Kitano:2002mt}.
substituting
\begin{align}
  \omega = & \frac{1}{8 \pi^2} G_F^2 m_\mu^5 \alpha^3 Z_{eff}^4/Z |F_p|^2 ||^2 + L \leftrightarrow R \\
  = & \frac{m_\mu^5 G_F^2 \alpha^3 Z_{eff}^4 |F_p|^2}{8 \pi^2 Z} \left( Z 
  \tilde{g}^{(p)}_{LV}\right) + L \leftrightarrow R
\end{align}
which is eq.~139 of \cite{Kuno:1999jp}.
For heavy nuclei it is important to include relativistic corrections.
We use method 2 of \cite{Kitano:2002mt} of determining the overlap integrals.

==> MuEGamma.tex <==
\section{$\mu \to e \gamma$}
Using \ref{eq:llgamma}
\begin{equation}
% eq. 51 of Hisano
  \Gamma(l_j \to l_i \gamma) = \frac{\alpha}{4} m_{l_j}^5 \left( \left|A_2^L\right|^2 + \left|A_2^R\right|^2 \right)
\end{equation}
\footnote{The calculation was also implemented in \texttt{FlexibleSUSY}.}

==> g-2.tex <==
\section{$g_\mu-2$}

The effective coupling o fermions to photon
\begin{equation}
\label{eq:llgamma}
  \mathcal{L}_{l l \gamma} = \bar{l}_i \left[ \gamma^\mu (A_L^1 P_L + A_R^1 P_R) + \imath m_j \sigma^{\mu \nu} (p_j - p_i)_\nu (A_2^L P_L + A^2_R P_R) \right] l_j A_\mu,
\end{equation}
where $P_{L/R} = (1 \mp \gamma^5)/2$ and $\sigma^{\mu \nu} = \imath/2 [\gamma^\mu, \gamma^\nu]$.

==> notatki.tex <==
\section*{Notes}

\subsection*{Translation between Kuno et al. and Hisano et al. conventions}
Lets start with the off-shell photon vertex in eq.~124 of ref.~\cite{Kuno:1999jp}
\begin{align}
M_{photonic} = & - e A_\mu^* \langle e^- | J(0) | \mu \rangle \nonumber \\
= & -e A_\mu^*(q) \bar{u}_e (p_e) [(f_{E0}(q^2) + \gamma^5 f_{M0}(q^2)) \gamma_\nu (g^{\mu \nu} - \frac{q^\mu q^\nu}{q^2}) \nonumber \\
\label{eq:KunoLag}
& + (f_{M1} (q^2) + \gamma^5 f_{E1}(q^2)) \frac{\imath \sigma_{\mu \nu} q^\nu}{m_\mu}] u_\mu (p_\mu)
\end{align}
and compare it with eq.~14 of \cite{Hisano:1995cp}
\begin{equation}
T = e \epsilon_{\alpha^*} \bar{u}_e [q^2 \gamma_\alpha (A_1^L P_L + A_2^R P_R) + m_\mu \imath \sigma_{\alpha \beta} q^\beta (A_2^L P_L + A_2^R P_R) ] u_\mu 
\end{equation}
Reordering eq.~\ref{eq:KunoLag} flips the sign of the $f_{M0}$ term
\begin{align*}
M_{photonic} = & -e A_\mu^*(q) \bar{u}_e (p_e) [\gamma_\nu (f_{E0}(q^2) - \gamma^5 f_{M0}(q^2))  (g^{\mu \nu} - \frac{q^\mu q^\nu}{q^2}) \\
& + \frac{\imath \sigma_{\mu \nu} q^\nu}{m_\mu} (f_{M1} (q^2) + \gamma^5 f_{E1}(q^2)) ] u_\mu (p_\mu)
\end{align*}
The relations between $f$ and $A$ coefficients are
\begin{align}
f_{E0} = & - q^2 (A_1^L + A_1^R) \approx m_\mu^2 (A_1^L + A_1^R)\\
f_{M0} = & - q^2 (A_1^L - A_1^R) \approx m_\mu^2 (A_1^L - A_1^R) \\
f_{M1} = & - \frac{1}{m_\mu^2} (A_2^L + A_2^R) \\
f_{E1} = & - \frac{1}{m_\mu^2} (A_2^R - A_2^L)
\end{align}
Using eqs.~140 and 141 of \cite{Kuno:1999jp} that transform photonic penguins into a contact vector-vector interactions
\begin{align}
\nonumber
\Delta g_{LV}^{(0)} =  \Delta g_{LV}^{(1)} =  &\frac{2\sqrt{2}\alpha \pi}{G_F m_\mu^2} (f_{E0} (-m_\mu^2) + f_{M1} (-m_\mu^2) + f_{M0} (-m_\mu^2) + f_{E1} (-m_\mu^2))\\
 = &\frac{4\sqrt{2}\alpha \pi}{G_F} (A_1^L - A_2^R) \\
\nonumber
\Delta g_{RV}^{(0)} = \Delta g_{RV}^{(1)}  =& \frac{2\sqrt{2}\alpha \pi}{G_F m_\mu^2} (f_{E0} (-m_\mu^2) + f_{M1} (-m_\mu^2) - f_{M0} (-m_\mu^2) - f_{E1} (-m_\mu^2))\\
= & \frac{4\sqrt{2}\alpha \pi}{G_F} (A_1^R - A_2^L)
\end{align}

% ------------------------------------------
\subsection*{\texttt{FlavourKit}}
The effective interaction of photon with fermions is written in \texttt{FlavourKit} as
\begin{equation}
L_{l l \gamma} = e \, \bar{l}_\beta \left[ \gamma^\mu \left(K_1^L P_L + K_1^R P_R \right) + i m_{l_\alpha} \sigma^{\mu \nu} q_\nu \left(K_2^L P_L + K_2^R P_R \right) \right] l_\alpha A_\mu + h.c.,
\end{equation}
But \texttt{FlavourKit} doesn't calculate the dipole operators $K_2$.
Instead, it calculates the following ones: $\mathbb{P}_{L/R} (\epsilon^* \cdot p_2)$ and $q^2 \mathbb{P}_{L/R} \gamma^\mu \epsilon_\mu^*$, as given by
\begin{verbatim}
AllOperators={
    {OA2lSL,Op[6] Pair[ec[3],k[1]]},
    {OA2lSR,Op[7] Pair[ec[3],k[1]]},
    {OA1L,Op[6,ec[3]] Pair[k[3],k[3]]},
    {OA1R,Op[7,ec[3]] Pair[k[3],k[3]]}
};
\end{verbatim}
According to \texttt{FormCalc}'s manual 6 is $\mathbb{P}_R$ and 7 is $\mathbb{P}_L$, so, for example, \texttt{OA2lSL} will contribute to dipole term with $P_R$ as given by the Gordon identity which reads
\begin{equation}
% https://www.fuw.edu.pl/~chank/qftoei_2.pdf
  \bar{u}(p_2) [(p_2 + p_1) \mathbb{P} + \imath \sigma^{\mu \nu}(p2-p1) \mathbb{P}] u(p_1) 
  = \bar{u}(p_2) [m_2 \gamma^\mu \mathbb{P} + m_1 \mathbb{P} \gamma_\mu ] u(p_1),
\end{equation}
where $\mathbb{P} \in \{\mathds{1}, \gamma^5, \mathbb{P_L}, \mathbb{P_R} \}$.
Neglecting $m_2$, which for us is the electron's mass gives
\begin{align}
  (p_2 + p_1)^\mu \bar{u}(p_2) \mathbb{P} u(p_1) = 
  \bar{u}(p_2) \imath \sigma^{\mu \nu} (p_1-p_2)_\nu \mathbb{P} u(p_1)
  + m_1 \bar{u}(p_2) \mathbb{P} \gamma_\mu u(p_1)
\end{align}

This is not what is done in \texttt{FlavourKit} according to Listing 6 in \cite{Porod:2014xia} where, for example, \texttt{K2L} $\sim$ \texttt{OA2lSL}.
This is also inconsistent with \texttt{GluonQQp} code in Listing 2 thereof where the projectors are flipped.
There's no reason why this should be different for gluons than for photons.
I've checked that this not a type in the preprint, but an actual thing in the code.
Also, it's still present even in the preprint released 2 years after the publication in the journal.
Also, the  \texttt{OA2lS} operator should contribute to \texttt{OA1} ones through the Gordon identity.
This is also not done anywhere in \texttt{SPheno}.

% -----------------------------------------------------
\subsection*{Box contributions}

The loop functions from Hyejung's code correspond to the following functions in \texttt{SPheno}
\begin{align}
I^\text{HJ}(x,y,z,t) &= \frac{1}{(4\pi)^2} D_0(x^2,y^2,z^2,t^2) \\
J^\text{HJ}(x,y,z,t) &= \frac{4}{(4\pi)^2} D_{00} (x^2,y^2,z^2,t^2)
\end{align}
% -------------------------------------------
%\subsection*{Derivation of the approximation for light nuclei}


